An Econometric Analysis of Large Flexible Cryptocurrency-mining Consumers in Electricity Markets

In recent years, power grids have seen a surge in large cryptocurrency mining firms, with individual consumption levels reaching 700MW. This study examines the behavior of these firms in Texas, focusing on how their consumption is influenced by cryptocurrency conversion rates, electricity prices, local weather, and other factors. We transform the skewed electricity consumption data of these firms, perform correlation analysis, and apply a seasonal autoregressive moving average model for analysis. Our findings reveal that, surprisingly, short-term mining electricity consumption is not directly correlated with cryptocurrency conversion rates. Instead, the primary influencers are the temperature and electricity prices. These firms also respond to avoid transmission and distribution network (T&D) charges - commonly referred to as four Coincident peak (4CP) charges - during the summer months. As the scale of these firms is likely to surge in future years, the developed electricity consumption model can be used to generate public, synthetic datasets to understand the overall impact on the power grid. The developed model could also lead to better pricing mechanisms to effectively use the flexibility of these resources towards improving power grid reliability.

==> hicss-packages.tex <==
\usepackage[letterpaper]{geometry}
\usepackage{hicss}
\usepackage{times}
\usepackage[none]{hyphenat}
\usepackage{url}
\usepackage{latexsym}
\usepackage{minted}
\usepackage{indentfirst}
\usepackage{graphicx}
\usepackage{multirow}
\usepackage{amsmath}
\usepackage[backend=biber, style=ieee]{biblatex}

% \graphicspath{{images/}}
% \usepackage[
%     style=apa,
%   ]{biblatex}
\addbibresource{sample.bib}

\usepackage[hang, flushmargin]{footmisc} % Load footmisc with options

% Set the margins for footnotes
\setlength{\footnotemargin}{10pt} % Adjust this value as needed
% \usepackage{hyperref} % Load hyperref
\usepackage{stfloats}
\usepackage{float}
% \usepackage{placeins} % Add this to your preamble


% % Reduce space between paragraphs
% \setlength{\parskip}{0.5em} % Adjust the value as needed (default is around 1em)
% \setlength{\parindent}{0em} % No indentation for paragraphs

% % Reduce space before and after equations
% \usepackage{amsmath}
% \setlength{\abovedisplayskip}{5pt} % Default is around 12pt
% \setlength{\belowdisplayskip}{5pt} % Default is around 12pt
% \setlength{\abovedisplayshortskip}{0pt}
% \setlength{\belowdisplayshortskip}{0pt}

% Reduce space before and after figures
\setlength{\floatsep}{3pt} % Space between floats
\setlength{\textfloatsep}{3pt} % Space between floats and text
\setlength{\intextsep}{3pt} % Space between in-text floats and text

% % Reduce space before and after sections
% \usepackage{titlesec}
% \titlespacing*{\section}{0pt}{1.5ex plus 1ex minus .2ex}{1ex plus .2ex}
% \titlespacing*{\subsection}{0pt}{1.25ex plus 1ex minus .2ex}{1ex plus .2ex}
% \titlespacing*{\subsubsection}{0pt}{1.25ex plus 1ex minus .2ex}{1ex plus .2ex}

% Package for more control over spacing
\usepackage{setspace}

% Custom commands to adjust spacing
\newcommand{\reduceparskip}{
    \setlength{\parskip}{0.5em}
    \setlength{\abovedisplayskip}{4pt}
    \setlength{\belowdisplayskip}{4pt}
    \setlength{\abovedisplayshortskip}{0pt}
    \setlength{\belowdisplayshortskip}{0pt}
    \setlength{\floatsep}{2pt}
    \setlength{\textfloatsep}{3pt}
    \setlength{\intextsep}{3pt}
}

\setstretch{0.943}
